A Space-Efficient Algebraic Approach to Robotic Motion Planning

We consider efficient route planning for robots in applications such as infrastructure inspection and automated surgical imaging. These tasks can be modeled via the combinatorial problem Graph Inspection. The best known algorithms for this problem are limited in practice by exponential space complexity. In this paper, we develop a memory-efficient approach using algebraic tools related to monomial testing on the polynomials associated with certain arithmetic circuits. Our contributions are two-fold. We first repair a minor flaw in existing work on monomial detection using a new approach we call tree certificates. We further show that, in addition to detection, these tools allow us to efficiently recover monomials of interest from circuits, opening the door for significantly broadened application of related algebraic tools. For Graph Inspection, we design and evaluate a complete algebraic pipeline. Our engineered implementation demonstrates that circuit-based algorithms are indeed memory-efficient in practice, thus encouraging further engineering efforts.

==> algorithms/search_prob_deprecated.tex <==
\begin{algorithm2e}[ht]
  \SetAlgoLined
  \KwInput{An instance $\mathcal{I}$ of \gi{},
  bounds of the optimal weight $\lo \leq \hi$,
  a failure count threshold $\theta$,
  and a success probability $p$ of an algorithm for \MLDshort.\\
  }
  \KwOutput{Optimal weight.}

  \BlankLine
  \tcp{Initialize lists.}
  Set $\alpha[i] \in \Z_{\geq 0}$ to $\alpha[i]=0$ for $\lo \leq i \leq \hi$.\;
  Set $\beta[i] \in \Z_{\geq 0}$ to $\beta[i]=0$ for $\lo \leq i \leq \hi$.\;
  Set $\gamma[i] \in \R_{\geq 0}$ to $\gamma[i]=0$ for $\lo \leq i \leq \hi$.\;

  Let $\hat{\ell} =\hi$.\tcp*{keep the original $\hi$}

  \BlankLine
  \While{$\lo < \hi$}{
    \If{$\sum_{\lo \leq i < \hi} \gamma[i]=0$}{
      Let $\ell \gets \lfloor \frac{\lo + \hi}{2} \rfloor$.\;
      Let $\gamma[\ell] \gets 1$.\;
    }
    \Else{
      Let $\ell \gets \argmax_{\lo \leq i < \hi} \gamma[i]$
    }
    \BlankLine
    Create a circuit $\C$ of $\mathcal{I}$ for $\ell$.\;
    Solve \MLDshort with $(\C, k)$ and get result \textsf{out}.\;

    \BlankLine
    \If{$\textnormal{\textsf{out}} = \true$}{
      \tcp{Increment success counter.}
      Let $\alpha[\ell] \gets \alpha[\ell] + 1$.\;
      Let $\hi \gets \ell$.\;
    }
    \Else{
      \tcp{Increment failure counter.}
      Let $\beta[\ell] \gets \beta[\ell] + 1$.\;

      \For{$i \gets \lo$ \KwTo $\ell$}{
        Let $a=\sum_{i \leq j < \hat{\ell}}\alpha[j]$.\;
        Let $b=\sum_{i \leq j < \hat{\ell}}\beta[j]$.\;
        \If {$\binom{a+b}{a}p^a (1-p)^b \leq (1-p)^\theta$}{
          \tcp{Concludes that $i$ is infeasible.}
          Let $\lo \gets i + 1$.\;
        }
      }

      \BlankLine
      \tcp{Distribute weights to higher half.}
      \If{$\ell \geq \lo$} {
        Let $\ell' \gets \lfloor \frac{\ell + 1 + \hi}{2} \rfloor$.\;
        \If{$\ell' < \hi$}{
          Let $\gamma[\ell'] \gets \gamma[\ell'] + p \cdot \gamma[\ell]$.\;
          Let $\gamma[\ell] \gets (1 - p)\cdot \gamma[\ell]$.\;
        }
      }
    }
  }
  \KwRet{$\hi$}\;
  \caption{\sprob}
  \label{alg:search-prob}
\end{algorithm2e}


% \begin{enumerate}
%   \item Initialize an integer array $c$ (failure counter) of size $\ell_\text{hi}$ (all initialized to $0$).
%   \item Initialize a real-valued array $w$ (weights) of size (all initialized to $0$).\YM{TODO: rename $w$ to another variable}
%   \item Do while $\ell < h$:
%   \begin{itemize}
%     \item If $\sum_{\ell \leq i < h} w[i] = 0$:
%     \begin{itemize}
%       \item Let $m \gets \lfloor (\ell + h)/2 \rfloor$ and $w[m]=1$.
%     \end{itemize}
%     \item Otherwise:
%     \begin{itemize}
%       \item Let\footnote{Pick a random one if there are ties.}
%        $m \gets \arg\max_{\ell \leq i < h} w[i]$.
%     \end{itemize}
%     \item Run the algorithm once with value $m$.
%     \begin{itemize}
%       \item If it succeeds, let $h \gets m$, continue from the beginning of the loop.
%       \item Let $c[m] \gets c[m] + 1$ (increment the failure counter).
%       \item If $\sum_{m \leq i < h} c[i] \geq q$,
%       then we are confident enough to state that $m$ is infeasible.
%       Let $\ell \gets m + 1$ and continue from the beginning of the loop.
%       \item Otherwise, let $m' \gets \lfloor (m + 1 + h)/2 \rfloor$.
%       \item If $m' = h$, then do nothing.
%       \item Otherwise, let $w[m'] \gets w[m'] + p \cdot w[m]$ and $w[m] \gets (1-p)w[m]$.
%     \end{itemize}
%   \end{itemize}
% \end{enumerate}


==> sections/21_acknowledgements.tex <==
\section*{Acknowledgements}
The authors thank Alan Kuntz for an introduction to the \gi{} problem and much assistance with the robotics data used in this paper, as well as Pål Grønås Drange for fruitful initial discussions.
This work was funded in part by the European Research Council (ERC) under the 
European Union's Horizon 2020 research and innovation programme (grant agreement No. 819416),
and by the Gordon \& Betty Moore Foundation's Data Driven Discovery Initiative
(award GBMF4560 to Blair D. Sullivan).
